Remote detectability from entanglement bootstrap I: Kirby's torus trick

Remote detectability is often taken as a physical assumption in the study of topologically ordered systems, and it is a central axiom of mathematical frameworks of topological quantum field theories. We show under the entanglement bootstrap approach that remote detectability is a necessary property; that is, we derive it as a theorem. Starting from a single wave function on a topologically-trivial region satisfying the entanglement bootstrap axioms, we can construct states on closed manifolds. The crucial technique is to immerse the punctured manifold into the topologically trivial region and then heal the puncture. This is analogous to Kirby's torus trick. We then analyze a special class of such manifolds, which we call pairing manifolds. For each pairing manifold, which pairs two classes of excitations, we identify an analog of the topological $S$-matrix. This pairing matrix is unitary, which implies remote detectability between two classes of excitations. These matrices are in general not associated with the mapping class group of the manifold. As a by-product, we can count excitation types (e.g., graph excitations in 3+1d). The pairing phenomenon occurs in many physical contexts, including systems in different dimensions, with or without gapped boundaries. We provide a variety of examples to illustrate its scope.

==> jm-tex-macros-no-hyperref.tex <==

%%%%% some colors
%\usepackage[usenames,dvipsnames]{xcolor}%http://en.wikibooks.org/wiki/LaTeX/Colors
\usepackage[]{xcolor}%http://en.wikibooks.org/wiki/LaTeX/Colors

%\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{amsmath,bm}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{amsfonts}         
\usepackage{fancybox}   
\usepackage{bbm}

%\usepackage{enumitem}

\usepackage{slashed}

\usepackage{yfonts} 
\usepackage{epstopdf}
\DeclareGraphicsRule{.tif}{png}{.png}{`convert #1 `dirname #1`/`basenam e #1 .tif`.png}

%\usepackage[bookmarks=true,colorlinks,linkcolor=red,urlcolor=blue,citecolor=blue]{hyperref}
%\usepackage[usenames]{color}

%\usepackage[usenames]{color}
\usepackage{wrapfig}
%\usepackage{hyperref}


%%from  Rudro Rana Biswas
%\usepackage[pagebackref,  % this puts links to the page numbers where refs appear
%pdftex, 
%bookmarks={false}, pdfauthor={John McGreevy}, pdftitle={Yay, physics!}]{hyperref}
%\hypersetup{colorlinks=true, 
%linkcolor=BrickRed, 
%citecolor=Violet, 
%filecolor=OliveGreen, 
%urlcolor=RoyalBlue, 
%filebordercolor={.8 .8 1}, 
%urlbordercolor={.8 .8 0}}%http://en.wikibooks.org/wiki/LaTeX/Hyperlinks
%%\usepackage[all]{hypcap}
%\usepackage{soul}%strike through text \st{} .  not in math mode.
%\setstcolor{Red}
%\usepackage{wrapfig}


\definecolor{darkgreen}{rgb}{0,0.4,0}
\definecolor{darkred}{rgb}{0.4,0,0}
\definecolor{darkblue}{rgb}{0,0,0.4}
\definecolor{lightblue}{rgb}{.6,.6,0.9}
\newcommand{\ttref}[1]{\textcolor{darkgreen}{\tiny{#1}}}
\newcommand{\blackcom}[1]{{\footnotesize{#1}}}
\newcommand{\greencom}[1]{\textcolor{darkgreen}{\footnotesize{#1}}}
\newcommand{\redcom}[1]{\textcolor{darkred}{\footnotesize{#1}}}
\newcommand{\bluecom}[1]{\textcolor{darkblue}{\footnotesize{#1}}}
\newcommand{\tttref}[2]{\textcolor{darkgreen}{
{#1, }\texttt{hep-th/{#2}}}}
\newcommand{\qcenter}[1]{\begin{center}{#1}\end{center}}
\def\bl{\textcolor{darkblue}}
\def\bluet{\textcolor{darkblue}}
\def\greent{\textcolor{darkgreen}}
\def\redt{\textcolor{darkred}}

%\newcommand{\blackcom}[1]{{\footnotesize{#1}}}

\newcommand{\cobl}{\color{darkblue}}

\newcommand{\cor}{\color{red}}
\newcommand{\cog}{\color{darkgreen}}
\newcommand{\cob}{\color{black}}

\definecolor{uglybrown}{rgb}{0.8,  0.7,  0.5}

\definecolor{palatinatepurple}{rgb}{0.41, 0.16, 0.38}

%%%%%%%%%%%%
% CHANGES SINCE HYPERREF SPLIT
\def\eqnfig#1#2{\parbox{#1}{
\includegraphics[height=#1]{#2}
}}
%\usepackage{mdframed}

\usepackage{framed}
\definecolor{shadecolor}{rgb}{0.90,0.90,0.90}

\def\CZ{{\cal Z}}

\usepackage{wasysym}




\definecolor{shadecolor}{rgb}{0.90,0.90,0.90}
\definecolor{DVcolor}{rgb}{0.95,  0.5,  0.2}
\definecolor{lightbluemuons}{rgb}{0.0,.65,1.0}

\definecolor{chartreuse}{rgb}{0.70, 1.00, 0.00}
\newcommand{\cogr}{\color{chartreuse}}
\newcommand{\colbl}{\color{lightbluemuons}}


%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%  TIKZ


\usepackage{tikz}
\usetikzlibrary{shapes}
\usetikzlibrary{trees}
\usetikzlibrary{snakes}
\usetikzlibrary{matrix,arrows}              % For commutative diagram
                                            % http://www.felixl.de/commu.pdf
\usetikzlibrary{positioning}                % For "above of=" commands
\usetikzlibrary{calc,through}               % For coordinates
\usetikzlibrary{decorations.pathreplacing}  % For curly braces
\usepackage[tikz]{bclogo}                   % For cute logo boxes
\usepackage{pgffor}                         % For repeating patterns

%\usetikzlibrary{decorations.pathmorphing}  % For Feynman Diagrams
\usetikzlibrary{decorations.markings}
\usetikzlibrary{intersections}              % For interesections

\usetikzlibrary{arrows,decorations.pathmorphing,backgrounds,positioning,fit,petri,automata,shadows,calendar,mindmap, graphs}
\usetikzlibrary{arrows.meta,bending}


% from flip tanedo.
% Based on:
% http://www.texample.net/tikz/examples/feynman-diagram/

\tikzset{
    % >=stealth', %% more traditional arrows, I don't like them
    vector/.style={decorate, decoration={snake}, draw},
    fermion/.style={postaction={decorate},
        decoration={markings,mark=at position .55 with {\arrow{>}}}},
    fermionbar/.style={draw, postaction={decorate},
        decoration={markings,mark=at position .55 with {\arrow{<}}}},
    fermionnoarrow/.style={},
    gluon/.style={decorate,
        decoration={coil,amplitude=4pt, segment length=5pt}},
    scalar/.style={dashed, postaction={decorate},
        decoration={markings,mark=at position .55 with {\arrow{>}}}},
    scalarbar/.style={dashed, postaction={decorate},
        decoration={markings,mark=at position .55 with {\arrow{<}}}},
    scalarnoarrow/.style={dashed,draw},
%
%%%     Special vectors (when you need to fine-tune wiggles)
%   provector/.style={decorate, decoration={snake,amplitude=2.5pt}, draw},
%   antivector/.style={decorate, decoration={snake,amplitude=-2.5pt}, draw},
%       electron/.style={draw=black, postaction={decorate},
%        decoration={markings,mark=at position .55 with {\arrow[draw=black]{>}}}},
%   bigvector/.style={decorate, decoration={snake,amplitude=4pt}, draw},
    vectorscalar/.style={loosely dotted,draw=black, postaction={decorate}},
}

\def\centerarc[#1](#2)(#3:#4:#5)% Syntax: [draw options] (center) (initial angle:final angle:radius)
    { \draw[#1] ($(#2)+({#5*cos(#3)},{#5*sin(#3)})$) arc (#3:#4:#5); }



%%%%%%%%%%%

\def\figblock#1#2#3#4{
\vskip.04in
\hskip-.24in
\parbox{#1\textwidth}{#3
}
\parfig{#2}{#4}
}


\def\ketbra#1#2{ | #1 \rangle\hskip-2pt\langle #2|}


\def\TT{{\bf T}}


\def\bn{{\bf n}}
\def\nn{{\bf n}}
\def\bb{{\bf b}}

\newcommand{\arxivlink}[1]{\htmladdnormallink{#1}{http://arxiv.org/abs/#1}}




%%%%%%%%%%%  new as of 2017-02-15





\def\futureNote#1{
{\footnotesize
\color{DVcolor}[#1]
}}






\def\sfE{\mathsf{E}}


\def\thump{\hfill$\blacksquare$}

%%%%%%%%%%% new as of 2016-03-16

\def\parsnip{-.22in}

\def\parfig#1#2{
\parbox{#1\textwidth}
{\includegraphics[width=#1\textwidth]{#2}}
}


%%%%%%%%%%%  new as of 2015-07-08


\def\angstrom{\buildrel{\circ} \over {\mathrm{A}}}

\def\mathmap#1#2#3#4{
#1 & \to &  #2 \cr 
#3 & \mapsto & #4 
}






%%%%%%%%%%%  new as of 2015-07-08

% from diptarka
\def\WIDERULE{\noindent\makebox[\linewidth]{\rule{\paperwidth}{0.4pt}}}


%%%%%%%% SLIDE SPECIFIC STUFF


%\newcommand{\headingslide}[1]{
%\begin{frame}{}
%\begin{center}
%\begin{shaded}
%{\huge #1}
%\end{shaded}
%\end{center}
%\end{frame}
%}


\newcommand{\headingslide}[1]{
%\begin{frame}{}
\frame{\begin{center}
\begin{shaded}
{\huge #1}
\end{shaded}
\end{center}}
}
%\end{frame}
%}


\def\partials#1#2#3{\( {\partial {#1} \over \partial {#2}} \)_{#3} }
%\def\subsubsubsection#1{{\bf\large #1}}
\def\subsubsubsection#1{{\bf #1}}
\def\eqbm{equilibrium}

\def\breakS{\vfill\eject}
% for posted version, you can remove pagebreaks by 
% \def\breakS{}



%%%%%% making revtex unnecessary:

%\textheight 22cm\textwidth 15.5cm
%\oddsidemargin 14pt\evensidemargin 0pt\topmargin -40pt
%\topmargin-20pt
%\def\baselinestretch{1.1}
%\addtolength{\parskip}{1ex}
%\jot=.5ex
%
%\setlength\arraycolsep{2pt}


\newcommand{\preprint}[1]{\begin{table}[t]  %%
             \begin{flushright}               %%
             {#1}                             %%
             \end{flushright}                 %%
             \end{table}}                     %%
%\renewcommand{\title}[1]{\vbox{\center\LARGE{#1}}\vspace{5mm}}
%\renewcommand{\author}[1]{\vbox{\center#1}\vspace{5mm}}
%\newcommand{\address}[1]{\vbox{\center\em#1}}
%\newcommand{\email}[1]{\vbox{\center\tt#1}\vspace{5mm}}


\newcommand{\pra}{Phys.~Rev.~A}
\newcommand{\prb}{Phys.~Rev.~B}
\newcommand{\prc}{Phys.~Rev.~C}
\newcommand{\prd}{Phys.~Rev.~D}
\newcommand{\pre}{Phys.~Rev.~E}
\newcommand{\prl}{Phys.~Rev.~Lett.}

%%%%%%%% things above here need to be adjusted in the template.

%%%%%%%%%%%% EQUATION NUMBERING  (must renew in appendix)
%\numberwithin{equation}{section}

%\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}




% the phantom dagger
\def\nd{{ \vphantom{\dagger}}}


\input epsf
\newcommand{\vev}[1]{\langle #1 \rangle}
\def\mapright#1{\!\!\!\smash{
\mathop{\longrightarrow}\limits^{#1}}\!\!\!}
\newcommand{\bigoint}{\displaystyle \oint}
%\newcommand{\ltimes}{\times \hspace{-6pt}
%\raisebox{.2ex}{\mbox{$\scriptscriptstyle |$}} \;}
\newlength{\extraspace}
\setlength{\extraspace}{2mm}
\newlength{\extraspaces}
\setlength{\extraspaces}{2.5mm}
\newcounter{dummy}
\addtolength{\abovedisplayskip}{\extraspaces}
\addtolength{\belowdisplayskip}{\extraspaces}
\addtolength{\abovedisplayshortskip}{\extraspace}
\addtolength{\belowdisplayshortskip}{\extraspace}
%\newcommand{\ee}{\end{equation}}
%\newcommand{\figuurnum}{\arabic{fignum}}
\newcommand{\figuur}[3]{
%\addtocounter{fignum}{1}
%\addcontentsline{lof}{figure}{\protect
%\numberline{\arabic{section}.\arabic{fignum}}{#3}}
\hspace{-3mm}{\it }\ %\figuurnum.
\begin{figure}[t]\begin{center}
\leavevmode\hbox{\epsfxsize=#2 \epsffile{#1.eps}}\\[3mm]
\medskip
\parbox{15cm}{%\small \bf Fig.\ %\figuurnum: 
#3}
\end{center} \end{figure}\hspace{-3.5mm}}
\newcommand{\figuurb}[3]{
%\addtocounter{fignum}{1}
%\addcontentsline{lof}{figure}{\protect
%\numberline{\arabic{section}.\arabic{fignum}}{#3}}
\hspace{-3mm}{\it }\ %\figuurnum.
\begin{figure}[ht]\begin{center}
\leavevmode\hbox{\epsfxsize=#2 \epsffile{#1.eps}}\\[3mm]
\parbox{11cm}{%\small \bf Fig.\ %\figuurnum: 
#3}
\end{center} \end{figure}\hspace{-3.5mm}}
\newcommand{\fig}{{\it}}% fig.}\ }




%\usepackage{textcomp}
%\usepackage{fontenc}
%\usepackage{bm}
%\usepackage{amsmath}
%\usepackage{yfonts}  % this is the one SS use
%\usepackage{mathbbol}
%\usepackage{arev}
%\usepackage{mbboard}
%\usepackage{devnagri}
%\usepackage{fc}
%\textwidth = 6.5 in
%\textheight = 9 in
%\oddsidemargin = 0.0 in
%\evensidemargin = 0.0 in
%\topmargin = 0.0 in
%\headheight = 0.0 in
%\headsep = 0.0 in
%\parskip = 0.2in
%\parindent = 0.1in


\def\be{\begin{equation}}
\def\ee{\end{equation}}



\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}









%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}{Definition}

\def\dbar{{\mathchar'26\mkern-12mu \dd}} 
\def\bdelta{ \slashed{\delta}}
\def\CU{{\cal U}}
%
%%MATH MACROS
%Greek letters and their bars
\def\ep{\epsilon}
\def\bep{\bar\epsilon}
\def\blam{\bar\lambda}
\def\bsig{\bar\sigma}
\def\bpsi{\bar\psi}
\def\bphi{\bar\phi}
\def\bp{\bar\partial}
\def\bthet{\overline \theta}
\def\Dbar{\overline D}
\def\bgam{\bar\gamma}
\def\p{\partial}
\def\tilp{\tilde\partial}
\def\eps{\epsilon}
\def\half{{1\over 2}}
\def\Tr{{{\rm Tr~ }}}
\def\tr{{\rm tr}}
\def\Re{{\rm Re\hskip0.1em}}
\def\Im{{\rm Im\hskip0.1em}}
\def\even{{\rm even}}
\def\odd{{\rm odd}}
\def\lcm{{\rm lcm}}
\def\diag{{\rm diag}}
\def\bra#1{{\langle}#1|}
\def\ket#1{|#1\rangle}
\def\bbra#1{{\langle\langle}#1|}
\def\kket#1{|#1\rangle\rangle}
\def\vev#1{\langle{#1}\rangle}
\def\Dslash{\rlap{\hskip0.2em/}D}
\def\dslash{\rlap{{\hskip0.08em/}}\partial}

\def\CA{{\cal A}}
\def\CB{{\cal B}}
\def\CC{{\cal C}}
\def\CD{{\cal D}}
\def\CE{{\cal E}}
\def\CF{{\cal F}}
\def\CG{{\cal G}}
\def\CH{{\cal H}}
\def\CI{{\cal I}}
\def\CJ{{\cal J}}
\def\CK{{\cal K}}
\def\CL{{\cal L}}
\def\CM{{\cal M}}
\def\CN{{\cal N}}
\def\CO{{\cal O}}%AEL
\def\CP{{\cal P}}
\def\CQ{{\cal Q}}
\def\CR{{\cal R}}
\def\CS{{\cal S}}
\def\CT{{\cal T}}
\def\CU{{\cal U}}
\def\CV{{\cal V}}
\def\CW{{\cal W}}
\def\CX{{\cal X}}%AEL
\def\CY{{\cal Y}}
\def\CZ{{\cal Z}}

\def\ad#1#2{{\delta\over\delta\sigma^{#1}(#2)}}
\def\ppt{{\partial\over\partial t}}
\def\comment#1{[#1]}
\def\nl{\hfill\break}
\def\a{\alpha}
\def\ta{\tilde\alpha}
\def\ap{\alpha'}
\def\sqap{\sqrt{\alpha'}}
\def\bA{\bar A}
\def\floor#1{{#1}}
\def\sgn{{\rm sgn\ }}
\def\I{{\rm I}}
\def\IA{{\rm IA}}
\def\II{\relax{I\kern-.10em I}}
\def\IIa{{\II}a}
\def\IIb{{\II}b}
\def\TeV{{\rm TeV}}
\def\hk{hyperk\"ahler\  }
\def\Hk{Hyperk\"ahler\  }
\def\cascade{{\cal A}}
%
%{\buildrel b \to i \over \longrightarrow}
\def\imp{$\Rightarrow$}
%\def\IZ{\relax\ifmmode\mathchoice
%{\hbox{\cmss Z\kern-.4em Z}}{\hbox{\cmss Z\kern-.4em Z}}
%{\lower.9pt\hbox{\cmsss Z\kern-.4em Z}}
%{\lower1.2pt\hbox{\cmsss Z\kern-.4em Z}}
%\else{\cmss Z\kern-.4emZ}\fi}
%\def\IZ{\relax{\rm Z\kern-.34em Z}}
\def\IZ{\mathbb{Z}}
\def\IB{\relax{\rm I\kern-.18em B}}
%\def\IC{{\relax\hbox{$\inbar\kern-.3em{\rm C}$}}}
\def\IC{\mathbb{C}}
\def\ID{\relax{\rm I\kern-.18em D}}
\def\IE{\relax{\rm I\kern-.18em E}}
\def\IF{\relax{\rm I\kern-.18em F}}
\def\IG{\relax\hbox{$\inbar\kern-.3em{\rm G}$}}
\def\IGa{\relax\hbox{${\rm I}\kern-.18em\Gamma$}}
\def\IH{\relax{\rm I\kern-.18em H}}
\def\II{\relax{\rm I\kern-.18em I}}
\def\IK{\relax{\rm I\kern-.18em K}}
%\def\IP{\relax{\rm I\kern-.18em P}}
\def\IP{\mathbb{P}}
%\def\IX{\relax{\rm X\kern-.01em X}}
%this doesn't work
\def\IX{{\bf X}}
%
\def\barom{\overline{\Omega}}
\def\barA{\bar{A}}
\def\jb{{\bar \jmath}}
\def\Hom{{\rm Hom}}
\def\inbar{\,\vrule height1.5ex width.4pt depth0pt}
\def\mod{{\rm\; mod\;}}
\def\ndt{\noindent}
\def\p{\partial}
\def\pab{\pb_{\bar A} }
\def\pb{{\bar \p}}
\def\pgp{\pb g g^{-1}}
\font\cmss=cmss10 \font\msss=cmss10 at 7pt
%\def\IR{\relax{\rm I\kern-.18em R}}
\def\IR{\mathbb{R}}
\def\pbar{\bar{\p}}
\def\qmvw{\CM_{\vec \zeta}(\vec v, \vec w) }
%i made these.
\def\sdtimes{\mathbin{\hbox{\hskip2pt\vrule
height 4.1pt depth -.3pt width .30pt\hskip-2pt$\times$}}}
%\def\simgt{\hskip0.05in\relax{ > 
%{\lower5.0pt\hbox{\kern-1.05em $\sim$}} } \hskip0.05in}
%\def\simlt{\hskip0.05in\relax{ <
%{\lower5.0pt\hbox{\kern-1.05em $\sim$}} } \hskip0.05in}
%\def\simlt{\hskip0.05in\relax{ 
%\raise3.0pt\hbox{ $<$
%{\lower5.0pt\hbox{\kern-1.05em $\sim$}} } \hskip0.05in}
%\def\simgt{\hskip0.05in\relax{ 
%\raise3.0pt\hbox{ $>$
%{\lower5.0pt\hbox{\kern-1.05em $\sim$}} }} \hskip0.05in}
\def\ker{{\rm ker\ }}
\def\cok{{\rm cok\ }}
\def\im{{\rm im\ }}
\def\ind{{\rm ind\ }}
\def\ub{{\bar{u}}}
\def\vol{{\rm vol}}
\def\Vol{{\rm Vol}}
\def\wb{{\bar{w}}}
\def\zb {{\bar{z}}}
\def\one {{\bf 1}}
\def\da{^{\dagger}}
\def\dpr{^{\prime\dagger}}
%
\def\BR{\IR}
\def\BZ{Z} % for now
\def\BP{\IP}
\def\BR{\IR}
\def\BC{\IC}
\def\BM{\QM}
\def\BH{\QH}
\def\BX{\QX}
%
\def\ls{l_s}
\def\ms{m_s}
\def\gs{g_s}
\def\lp10{\ell_p^{10}}
\def\lp11{\ell_p^{11}}
\def\R11{R_{11}}
\def\mb{{m_{\rm brane}}}
\def\vb{{v_{\rm brane}}}
%
\def\brs{Q_{{\rm B}}}
\def\brsb{\bar{Q}_{{\rm B}}}
\def\dels{\delta_{{\rm S}}}
\def\delb{\delta_{{\rm B}}}
\def\zb{\bar{z}}
\def\frac#1#2{{#1 \over #2}}
\def\epb{\bar{\epsilon}}
\def\tts{{\rm tt}{}^\ast}
\def\ch{{\rm ch}}
\def\td{{\rm Td}}
\def\ahat{\hat{A}}
\def\cft#1{{\rm CFT_{#1}}}
\def\dS{\partial \Sigma}
%\def\ni{\noindent}
\def\imt{{\rm Im} \tau}
\def\mfl{ (-1)^{F_L}}
\def\mfr{ (-1)^{F_R}}

\def\up{\uparrow}
\def\down{\downarrow}

\def\norm#1{\vrule\hskip-1.2pt \vrule \hskip1.2pt #1  \hskip1.2pt \vrule\hskip-1.2pt \vrule}
\def\norm#1{|\hskip-1.5pt | \hskip1.5pt #1  \hskip1.5pt |\hskip-1.5pt |}
%$ \norm{A}$

%identity operator from doyon-fonseca
\def\Ione{\hbox{$1\hskip -1.2pt\vrule depth 0pt height 1.53ex width 0.7pt
                  \vrule depth 0pt height 0.3pt width 0.12em$}}


\def\norm#1{\vrule\hskip-1.2pt \vrule \hskip1.2pt #1  \hskip1.2pt \vrule\hskip-1.2pt \vrule}
\def\norm#1{|\hskip-1.5pt | \hskip1.5pt #1  \hskip1.5pt |\hskip-1.5pt |}
%$ \norm{A}$


\def\thetafunction#1#2#3#4{
\vartheta\left[\matrix{ #1 \cr #2} \right] (#3 |#4)}



%% from the topological vertex paper


%%                              TABLEAUX.TEX
%%      This  macro file is for producing a ``Young Tableau'' which is
%%      an array of little squares sometimes used in mathematical physics.
%%      For instance, the command $\tableau{6 3 2}$ will produce a tableau
%%      with 6 squares in the top row, 3 in the next, and 2 in the last.
%%                                  OOOOOO
%%      This tableau will look like OOO    but made of squares instead of O's.
%%                                  OO
%%      Any number of rows may be present, each having a nonzero number of
%%      squares.
%%
%%      A tableau is math mode material, so use $ or $$ to enclose it.
%%
%%      The size and line-thickness of the little boxes are controlled by the
%%      dimension parameters --
%%              \tableauside=1.0ex              %(size)
%%              \tableaurule=0.4pt              %(line-thickness)
%%      Change them if you want.
%%
%%                                                      -- Doug Eardley 9/19/8%%
%%
\newdimen\tableauside\tableauside=1.0ex
\newdimen\tableaurule\tableaurule=0.4pt
\newdimen\tableaustep
\def\phantomhrule#1{\hbox{\vbox to0pt{\hrule height\tableaurule width#1\vss}}}
\def\phantomvrule#1{\vbox{\hbox to0pt{\vrule width\tableaurule height#1\hss}}}
\def\sqr{\vbox{%
  \phantomhrule\tableaustep
  \hbox{\phantomvrule\tableaustep\kern\tableaustep\phantomvrule\tableaustep}%
  \hbox{\vbox{\phantomhrule\tableauside}\kern-\tableaurule}}}
\def\squares#1{\hbox{\count0=#1\noindent\loop\sqr
  \advance\count0 by-1 \ifnum\count0>0\repeat}}
\def\tableau#1{\vcenter{\offinterlineskip
  \tableaustep=\tableauside\advance\tableaustep by-\tableaurule
  \kern\normallineskip\hbox
    {\kern\normallineskip\vbox
      {\gettableau#1 0 }%
     \kern\normallineskip\kern\tableaurule}%
  \kern\normallineskip\kern\tableaurule}}
\def\gettableau#1 {\ifnum#1=0\let\next=\null\else
  \squares{#1}\let\next=\gettableau\fi\next}

\tableauside=1.0ex
\tableaurule=0.4pt


%% from shiraz


\font\smallrm=cmr8
 \def\app#1#2{\global\meqno=1\global\subsecno=0\xdef\secsym{\hbox{#1.}}
 \bigbreak\bigskip\noindent{\bf Appendix.}\message{(#1. #2)}
 \writetoca{Appendix {#1.} {#2}}\par\nobreak\medskip\nobreak}
 %
 %       \eqn\label{a+b=c}       gives displayed equation, numbered
 %                               consecutively within sections.
%     \eqnn and \eqna define labels in advance (of eqalign?)
 %
 \def\eqnn#1{\xdef #1{(\secsym\the\meqno)}\writedef{#1\leftbracket#1}%
 \global\advance\meqno by1\wrlabeL#1}
 \def\eqna#1{\xdef #1##1{\hbox{$(\secsym\the\meqno##1)$}}
 \writedef{#1\numbersign1\leftbracket#1{\numbersign1}}%
 \global\advance\meqno by1\wrlabeL{#1$\{\}$}}
 \def\eqn#1#2{\xdef #1{(\secsym\the\meqno)}\writedef{#1\leftbracket#1}%
 \global\advance\meqno by1$$#2\eqno#1\eqlabeL#1$$}

%\def\IZ{\relax\ifmmode\mathchoice
% {\hbox{\cmss Z\kern-.4em Z}}{\hbox{\cmss Z\kern-.4em Z}}
% {\lower.9pt\hbox{\cmsss Z\kern-.4em Z}}
% {\lower1.2pt\hbox{\cmsss Z\kern-.4em Z}}\else{\cmss Z\kern-.4em Z}\fi}



\global\newcount\itemno \global\itemno=0
\def\itemized{\global\itemno=0\bigbreak\bigskip\noindent}
\def\itemaut#1{\global\advance\itemno by1\noindent\item{\the\itemno.}#1}

%\itemized
%\itemaut{First this.}
%\itemaut{Then that.}


\def\bs{\backslash}
\def\bfe{{\bf e}}

\def\del{\partial}

\def\({\left(}
\def\){\right)}

\def\sidebarb{\color{darkblue}
\vskip.2in
\hrule 
}

\def\sidebare{
\vskip.2in
\hrule 
\cob
}


\def\ppi{\boldsymbol{\pi}}
\def\pphi{\boldsymbol{\phi}}
%\def\pphi{\phi}
\def\grad{\vec \nabla}
\def\vB{\vec B}
\def\vE{\vec E}
\def\vA{\vec A}
\def\vAA{ \vec{\bf A}}
\def\vEE{{{\vec {\bf E}}}}
\def\vBB{{\vec {\bf B}}}

\def\cc{{\bf c}}

\def\ii{{\bf i}}


\def\CK{{\cal K}}
\def\xx{{\bf x}}
\def\yy{{\bf y}}

\def\dd{\text{d}}

\def\pp{{\bf p}}
\def\aa{{\bf a}}
\def\qq{{\bf q}}

\def\AA{{\bf A}}
\def\BB{{\bf B}}
\def\EE{{\bf E}}
\def\HH{{\bf H}}
\def\KK{{\bf K}}
\def\JJ{{\bf J}}
\def\MM{{\bf M}}
\def\NN{{\bf N}}
\def\PP{{\bf P}}
\def\QQ{{\bf Q}}
\def\RR{{\bf R}}
\def\SS{{\bf S}}


\def\UU{{\bf U}}
\def\VV{{\bf V}}
\def\WW{{\bf W}}
\def\rrho{{\boldsymbol\rho}}
\def\ssigma{{\boldsymbol\sigma}}
\def\ttau{{\boldsymbol\tau}}
\def\SSigma{{\boldsymbol\Sigma}}
\def\Prob{\text{{\bf Prob}}}

 \def\XX{{\bf X}}
 \def\ZZ{{\bf Z}}
\def\YY{{\bf Y}}
\def\cnot{\CC_\text{not}}

\def\DDD{\boldsymbol{\Delta}}

%Approximately less than operators:
\def\lsim{\mathrel{\mathstrut\smash{\ooalign{\raise2.5pt\hbox{$<$}\cr\lower2.5pt\hbox{$\sim$}}}}}
\def\gsim{\mathrel{\mathstrut\smash{\ooalign{\raise2.5pt\hbox{$>$}\cr\lower2.5pt\hbox{$\sim$}}}}}

\def\MSbar{\overline{\text{MS}}}


%A leftright arrow which acts like \vec:
\def\overleftrightarrow#1{\vbox{\ialign{##\crcr
     $\leftrightarrow$\crcr\noalign{\kern-0pt\nointerlineskip}
     $\hfil\displaystyle{#1}\hfil$\crcr}}}
     
     \def\overleftarrow#1{\vbox{\ialign{##\crcr
     $\leftarrow$\crcr\noalign{\kern-0pt\nointerlineskip}
     $\hfil\displaystyle{#1}\hfil$\crcr}}}


%%ENGLISH MACROS
\def\eg{{\it e.g.}}
\def\ie{{\it i.e.}}
\def\cf{{\it c.f.}}
\def\etal{{\it et. al.}}
\hyphenation{Di-men-sion-al}

%%% additions new to 239a


\def\hh{{\bf h}}

\def\gSO{\textsf{SO}}
\def\gG{\textsf{G}}

\def\gO{\textsf{O}}
\def\gSU{\textsf{SU}}
\def\gU{\textsf{U}}
\def\gS{\textsf{S}}


\def\gs{\text{gs}}




\usepackage[yyyymmdd,hhmmss]{datetime}

\renewcommand{\theequation}{\arabic{equation}}
\newif{\ifeq}           % defines a new condition @eq tested by the conditional \ifeq
\eqtrue                 % if uncommented, declares @eq to be true
%\eqfalse               % if uncommented, declares @eq to be false
                                %
                                % to use this, wrap text with the conditional, eg:
                                %
                                % \ifeq
                                % SHOW THIS IFF \eqtrue HAS BEEN DECLARED
                                % \fi

\def\answer#1
{
\ifeq
\textcolor{darkblue}{#1}
\fi
}

\textheight 22cm
\textwidth 15.5cm
\oddsidemargin 0pt\evensidemargin 0pt
%\oddsidemargin 14pt\evensidemargin 0pt
%\topmargin -40pt
\topmargin-30pt
%\bottommargin0pt
\def\baselinestretch{1.1}
%\addtolength{\parskip}{1ex}
\jot=.5ex

\newcounter{lecturecounter}
% \addtocounter{lecturecounter}{19}


%\newcounter{lecturecounter}
%%[counter]
\newcommand{\Lec}{
\stepcounter{lecturecounter}
\color{blue}
\hfill[End of Lecture \arabic{lecturecounter}]
\cob
% \addtocounter{lecturecounter}{1}
}


%\newcounter{bar}
%\newcommand{\Lec}{%
%        \stepcounter{bar}%
%        \thebar}


%% SKIP TO HERE

%\renewcommand{\thesubsection}{(\alph{subsection})}
%\renewcommand{\thesubsection}{(\roman{subsection})}
%\newpage
%\setcounter{page}{1}
%\def\chapternumber{1}
%\renewcommand{\thesection}{\chapternumber}
%\renewcommand{\thepage}{\chapternumber-\arabic{page}}

%\title{Lecture Notes}
%% Lecture Notes}
%%Chapter \chapternumber: }
%\author{Lecturer: McGreevy
%%\footnote
%%{}
%}
%\date{{\tiny Last updated: \today, \currenttime}
%}
%\begin{document}
%\maketitle
%
%%\vfill
%
%\renewcommand{\contentsname}{}
%%\vskip-.5in
%%\breakS
%
%\tableofcontents
%
%\breakS
%
%\section{}
%\end{document}

